Tuning of Mixture-of-Experts Mixed-Precision Neural Networks

Deep learning has become a useful data analysis method, however mainstream adaption in distributed computer software and embedded devices has been low so far. Often, adding deep learning inference in mainstream applications and devices requires new hardware with signal processors suited for convolutional neural networks. This work adds new data types (quantized 16-bit and 8-bit integer, 16-bit floating point) to Caffe in order to save memory and increase inference speed on existing commodity graphics processors with OpenCL, common in everyday devices. Existing models can be executed effortlessly in mixed-precision mode. Additionally, we propose a variation of mixture-of-experts to increase inference speed on AlexNet for image classification. We managed to decrease memory usage up to 3.29x while increasing inference speed up to 3.01x on certain devices. We demonstrate with five simple examples how the presented techniques can easily be applied to different machine learning problems. The whole pipeline, consisting of models, example python scripts and modified Caffe library, is available as Open Source software.

==> results.tex <==
\chapter{Results}
\label{ch:results}

\section{Introduction}
In this chapter, the results of training the models from Chapter \ref{ch:models} are presented.

The evaluation is based on:
\begin{itemize}
	\item Two data sets (DS1 and DS2: see Chapter \ref{ch:datasets}).
	\item Three models (SK, U, USK: see Chapter \ref{ch:models}).
	\item Two training loss functions (Softmax and Malis).
	\item One processing loss function (Softmax).
	\item Three training configurations (Softmax, Malis and Softmax + Malis).
	\item 10'000 training iterations per configuration, respectively 20'000 for combined training.
	\item Three error objectives (rand, warping and pixel error).
\end{itemize}

The amount of training iterations was chosen so that training of all 18 combinations was feasible during one week on two AMD W9100 GPUs, providing a total of \SI{10}{TFLOP/s} \cite{W9100Whitepaper}.\\
The training data is not very large in both cases (see Chapter \ref{ch:datasets}) and thus the loss always converged in under 10'000 iterations for each training method. It is possible that some trainings did overfit as no early stopping was applied. Technically, the networks did not get to see the same amount of examples during training even though the iterations are the same, as the chosen output sizes of each network were set differently. However, due to gradient accumulation, different learning rates and weight initialization it is hard to estimate the effect of the amount of labels seen. As all networks converged to a stable loss, it should negligible.

\section{Analysis on DS1}
\label{sec:ds1analysis}

\subsection{Training}
The training parameters used on DS1 were set to not use the error masking functionality. Masking usually gives thicker membrane (background) labels when used with Softmax by balancing out the amount of background error against foreground (cell interior) error.

Malis loss was run without using a patch prior for preferring training patches based on their label histogram. Softmax loss on the other hand was used with the patch prior enabled. This is justified by the different characters of the loss functions: Softmax computes a per-pixel error while Malis gives errors at problematic pixels only, which can be very concentrated on a few pixels (see Section \ref{sec:malisloss}).

In the patch pre-processing step, the images were enhanced with CLAHE (contrast limited adaptive histogram equalization) and normalized in the range of $[-1.0,1.0]$.

To get more training data, the images were blurred with a randomly chosen 5 by 5 Gaussian kernel. The training patches were also rotated to multiples of \ang{90} and mirrored randomly (horizontal and vertical).

Details of the pre-processing and label priors are described in Chapter \ref{ch:caffeneuraltool}. The exact training parameters are stored as prototxt configuration in the Caffe Neural Models repository \cite{CaffeNeuralModels}.

Interestingly, it was not possible to start training of the SK network with Malis loss directly. The loss did not converge, and the output feature maps drifted to being classified as only foreground or only background. Therefore, the weights of the network in \textit{Malis only}-training were initialized using 4000 iterations of Softmax training first. This was the lowest number of iterations where the training converged to a small loss afterwards. The other network architectures did not show such a behavior and trained well when starting with Malis directly.\\
This is related to weight initialization as well as the fact that Malis works better on bigger training patch sizes. Training of SK was limited to 128 by 128 pixels output, which is much less context for Malis to work on than with USK and U with 512 by 512 and 388 by 388 pixels respectively.

\subsection{Numerical}

\begin{table}[H]
\begin{center}
	\begin{tabular}{|l|l|l|r|r|r|}
		\hline
		\textbf{Rank} & \textbf{Network} & \textbf{Loss Function} & \textbf{Rand} & \textbf{Warping} & \textbf{Pixel}\\\hline
		1. & USK & Softmax + Malis & \textbf{0.031251499} & 0.000423193 & 0.040650392\\\hline
		2. & SK & Softmax + Malis & 0.043871103 & \textbf{0.000324726} & 0.052724789\\\hline
		3. & USK & Malis & 0.045955948 & 0.000578165 & 0.058407081\\\hline
		4. & U & Softmax + Malis & 0.050799468 & 0.000487328 & 0.044159558\\\hline
		5. & SK & Malis & 0.063852001 & 0.000386953 & 0.055678171\\\hline
		6. & USK & Softmax & 0.067068677 & 0.000418186 & \textbf{0.030634890}\\\hline
		7. & U & Malis & 0.078736573 & 0.000520945 & 0.059127919\\\hline
		8. & U & Softmax & 0.091736036 & 0.000595331 & 0.033451667\\\hline
		9. & SK & Softmax & 0.123334489 & 0.000549316 & 0.034416625\\\hline
	\end{tabular}
	\captionof{table}{DS1 error evaluation (lower is better).}
	\label{tab:ds1ranking}
\end{center}
\end{table}

\newpage
Explanations for the Tables \ref{tab:ds1ranking} and \ref{tab:ds2ranking}:
\begin{itemize}
	\item Rank: The internal ranking, as indicated by the rand error.
	\item Loss Function: Softmax indicates 10'000 iterations with the Softmax loss function. Malis indicates 10'000 iterations with the Malis loss function. When both are indicated, the training was executed with 10'000 Softmax and then 10'000 Malis training iterations.
	\item Rand, warping and pixel: Error metrics, as proposed by Jain \etal \cite{Jain2010} and used in the ISBI 2012 challenge \cite{ISBI2012}. A script for evaluation is available for Fiji \cite{fijiscript} in the Caffe Neural Models repository \cite{CaffeNeuralModels}.
\end{itemize}

The ranking on data set DS1 is as expected: Taking the average rank, USK-Net performs better than SK-Net, which is more precise than U-Net.\\
The same goes for training methods: Using Softmax + Malis minimizes the rand error better than using Malis only, and Softmax outperforms Malis on pixel precision.
On one hand, this is because the Malis criterion improves the rand error by penalizing merge and split errors. On the other hand, training with Malis will also decrease the pixel accuracy, which can be seen when inspecting the result visually.\\
As Softmax training initializes the networks better than Malis, the best training method is to start with Softmax and then transit to Malis for fine tuning.\\
Obviously, the USK network architecture performed best on both pixel accuracy and rand error. Only for the warping error, the much slower SK-Net (see Section \ref{sec:labelthroughput}) performs best.

\subsection{Visual}
The visual analysis is based on the image number 2 of the DS1 stack (see Section \ref{sec:dataset1}). It includes a glia cell (Figure \ref{fig:ds1araw}, label A) which is considered as background. The thickness of it makes it harder to label correctly, especially with Malis loss.

\begin{figure}[H]
	\center
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_raw_P.png}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_label_P.png}
	\end{subfigure}%
	\caption{DS1 ssTEM raw and corresponding ground truth, 1024 by 1024 pixels (Source: ssTEM \cite{DS1ssTEM}, \cite{CaffeNeuralModels}).}
	\label{fig:ds1araw}
\end{figure}

\begin{figure}[H]
	\center
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_SK_S_P.png}
		\caption{SK network, Softmax.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_U_S_P.png}
		\caption{U network, Softmax.}
	\end{subfigure}%
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_USK_S_P.png}
		\caption{USK network, Softmax.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_SK_M_P.png}
		\caption{SK network, Malis.}
	\end{subfigure}%
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_U_M_P.png}
		\caption{U network, Malis.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_USK_M_P.png}
		\caption{USK network, Malis.}
	\end{subfigure}%
	\newline
	\caption{Visual comparison of all results in Table \ref{tab:ds1ranking}.}
\end{figure}

\begin{figure}[H]
	\ContinuedFloat
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_SK_SM_P.png}
		\caption{SK network, Softmax + Malis.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_U_SM_P.png}
		\caption{U network, Softmax + Malis.}
	\end{subfigure}%
	\pagebreak
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.18]{data/ds1a_USK_SM_P.png}
		\caption{USK network, Softmax + Malis.}
	\end{subfigure}%
	\caption{Visual comparison of all results in Table \ref{tab:ds1ranking}.}
	\label{fig:ds1visualresults}
\end{figure}
Explanation to the labels in Figure \ref{fig:ds1visualresults}:
\begin{enumerate}[label=(\Alph*)]
	\item Glia cell that should be considered background. Malis loss does focus on separating foreground objects, so this part gets only labeled correctly in the trainings that use Softmax only (a, b and c).
	\item Diffuse membrane with light texture, which is hard to separate from cell interior. The separation is correct only in SK + Malis (d), while all other configurations lead to connected cells, although all trainings with Malis (d to i) show uncertainty, which could be sufficient to segment correctly. Diffuse parts are always on the edge of being pushed to foreground or background, which makes the segmentation fragile.
	\item Membrane with close proximity to a mitochondrion. Except for U networks that have been trained with Softmax (b and h), this gets labeled correctly. The downsampling of U-Net is sub-optimal here when pixel error (without scaling) instead of foreground separation is the training objective.
	\item Same case as label C, but here the mitochondrion is labeled with high certainty by all networks, leading to mislabeling of the nearby membrane.
	\item Removing an isolated mitochondrion with high certainty. The USK network (c and i) performed best on this task. Malis trainings are usually worse, again because Malis does not focus on pixel accuracy.
	\item Mitochondrion with long, thin structure. It consequently leads to a wrong classification as membrane because of its shape. This is not an issue, as isolated misclassifications within a cell can be rejected on a higher level when reconstructing the connectome.
	\item Mitochondrion close to the image border. As the training and classification uses border mirroring to make up for the missing context, it can lead to more errors near the border, independent of the network architecture.
	\item Same case as label G. Softmax + Malis on USK-Net performed best on removing the mitochondria on E, F, G and H.
	\item Diffuse membrane with a dark texture. It is expected that this gets completely classified as membrane. However, this was not the case on all networks and trainings. The worst case applies on U-Net (b and h), where the cells are almost connected.
\end{enumerate}

As expected, membranes get labeled thinner with Malis as this error criterion is stopping to provide loss at membranes as soon as two cells are sufficiently separated (see Section \ref{sec:malisloss}). Even though the separation border is thin, training with Malis separates cells very well and scores best on both DS1 (Table \ref{tab:ds1ranking}) and DS2 (Table \ref{tab:ds2ranking}).

The visual results match the numerical evaluation. USK performs best on pixel error with Softmax and best on rand error with Softmax + Malis. However, when using Softmax, there is not a huge difference in pixel error and visual results between the networks. Malis does not work very well on SK networks (d), leaving a lot of uncertainty in the prediction. It can still be a good segmentation, as thresholding of gray scale values can be applied. The numeric evaluation \cite{fijiscript} does test different thresholds, which is why the score is rather good (see Table \ref{tab:ds1ranking}) despite the uncertainty.

\section{Analysis on DS2}
\label{sec:ds2analysis}

\subsection{Training}
Training on DS2 was similar to training on DS1. The main difference is that the patch prior was not used on both Softmax and Malis. Instead, the error masking was enabled when using Softmax, which gives thicker borders. This is motivated by having input images which are slightly more blurred and thus the cell membranes are less sharp and harder to distinguish from cell interior.

Here, the SK network already converged using 2000 training iterations of Softmax before switching over to Malis. Starting with Malis directly was also not possible.

\subsection{Numerical}

\begin{table}[H]
\begin{center}
	\begin{tabular}{|l|l|l|r|r|r|}
		\hline
		\textbf{Rank} & \textbf{Network} & \textbf{Loss Function} & \textbf{Rand} & \textbf{Warping} & \textbf{Pixel}\\\hline
		1. & SK & Softmax + Malis & \textbf{0.060110507} & \textbf{0.000495529} & 0.106053779\\\hline
		2. & USK & Malis & 0.085927407 & 0.000848007 & 0.110390552\\\hline
		3. & SK & Malis & 0.086975487 & 0.000572968 & 0.107365432\\\hline
		4. & SK & Softmax & 0.087380844 & 0.000585556 & 0.075981492\\\hline
		5. & U & Softmax + Malis & 0.097356122 & 0.000940704 & 0.101856259\\\hline
		6. & USK & Softmax & 0.102450251 & 0.000851440 & \textbf{0.073163943}\\\hline
		7. & U & Malis & 0.121984927 & 0.001038742 & 0.111951817\\\hline
		8. & USK & Softmax + Malis & 0.128440534 & 0.000858688 & 0.101919859 \\\hline
		9. & U & Softmax & 0.148045042 & 0.001293564 & 0.083922396\\\hline
	\end{tabular}
	\captionof{table}{DS2 error evaluation (lower is better).}
	\label{tab:ds2ranking}
\end{center}
\end{table}

Interestingly, the USK-Net with Softmax + Malis loss training performs unexpectedly worse on the dataset DS2 than on DS1, where it performed best.
What is common for both DS1 and DS2 is that the USK network combined with Softmax training performs best on the pixel error.
Overall, this data set has a ranking much harder to explain than on DS1. Visual inspection reveals that the USK-Net was often overconfident when labeling the cell interior, which connected cells that should be separated. On the DS1 data set, this did not happen.

\begin{table}[H]
\begin{center}
	\begin{tabular}{|l|r|r|r|}
		\hline
		\textbf{Network} & \textbf{Rand} & \textbf{Warping} & \textbf{Pixel}\\\hline
		U & 0.0382 & 0.000353 & 0.0611\\\hline
	\end{tabular}
	\captionof{table}{(Source: Ronneberger \etal \cite{2015arXiv150504597R}).}
	\label{tab:unetres}
\end{center}
\end{table}
Finally, the results of U-Net obtained by Ronneberger \etal \cite{2015arXiv150504597R} (Table \ref{tab:unetres}) could not be reached, probably due to having used less transformations to extend the training data. It is not inherently clear if the U network would perform better than SK and USK given the bigger training data set.

Ideas to improve training include:
\begin{itemize}
	\item Weight maps to scale the loss instead of only masking it.
	\item Add elastic deformations, shifting and scaling instead of only rotation and mirroring to increase the amount of training data.
	\item Experiment with different loss functions than Malis and Softmax, or alternate between them during training.
\end{itemize}

\subsection{Visual}

The visual analysis is based on the image number 16 of the DS2 test stack (see Section \ref{sec:dataset2}).

\begin{figure}[H]
	\center
	\includegraphics[scale=0.37]{data/ds2a_raw_P.png}
	\caption{DS1 raw image, 512 by 512 pixels (Source: ISBI challenge \cite{ISBI2012}, \cite{CaffeNeuralModels}).}
	\label{fig:ds2araw}
\end{figure}

Explanation to the labels in Figure \ref{fig:ds1visualresults}:

The visual results of Softmax training (a to c) have thicker membrane labels than on DS1. This is because the error masking was enabled here and, as a result, the network has seen the same amount of error pixels for both foreground and background.

\begin{enumerate}[label=(\Alph*)]
	\item A bright spot, which is an error in the electron microscopy image. The membrane affected by it is misclassified by all networks and trainings. The local contrast enhancement with CLAHE did not help here. 
	\item Mitochondrion with close proximity parallel to a cell membrane. The USK network removes the membrane with all trainings (c, f and i). U-Net (b, e and h) performs a little better, but still merges the two cells. Only the SK network does it correctly (a, d and g), but has some uncertainty on the mitochondrion instead (d).
	\item Diffuse section of a cell membrane. This is not an issue on most training/architecture combinations, except for U-Net with Softmax (b and h).
	\item Oriented structures, even when faint, are partially labeled as membrane when sharp enough and of similar thickness as the membrane. This is no issue when isolated within the cell and not cutting through a cell that should be connected. With convolutional networks, this is hard to impossible to label correctly. It would require more high level knowledge of the object, such as if the predicted membrane is enclosing a cell or not.
\end{enumerate}

\begin{figure}[H]
	\center
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_SK_S_P.png}
		\caption{SK network, Softmax.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_U_S_P.png}
		\caption{U network, Softmax.}
	\end{subfigure}%
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_USK_S_P.png}
		\caption{USK network, Softmax.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_SK_M_P.png}
		\caption{SK network, Malis.}
	\end{subfigure}%
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_U_M_P.png}
		\caption{U network, Malis.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_USK_M_P.png}
		\caption{USK network, Malis.}
	\end{subfigure}%
	\newline
	\caption{Visual comparison of all results in Table \ref{tab:ds2ranking}.}
\end{figure}

\begin{figure}[H]
	\ContinuedFloat
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_SK_SM_P.png}
		\caption{SK network, Softmax + Malis.}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_U_SM_P.png}
		\caption{U network, Softmax + Malis.}
	\end{subfigure}%
	\pagebreak
	\newline
	\begin{subfigure}{0.5\textwidth}
		\center
		\includegraphics[scale=0.37]{data/ds2a_USK_SM_P.png}
		\caption{USK network, Softmax + Malis.}
	\end{subfigure}%
	\caption{Visual comparison of all results in Table \ref{tab:ds2ranking}.}
\end{figure}

\begin{enumerate}[label=(\Alph*), resume]
	\item Diffuse mitochondrion. The same situation as with B applies. Especially U- and USK-Net with Softmax training (b and c) get it wrong.
	\item Diffuse cell interior that is similar to the membrane texture. All networks see a membrane connection through this area. In the training data there are some examples of diffuse membranes, so the networks have slightly overfitted on the training data for this case.
\end{enumerate}


==> typography.tex <==
\chapter{Typography}


\section{Punctuation}

\begin{Rule}
  Use opening (`) and closing (') quotation marks correctly.
\end{Rule}

In \LaTeX, the closing quotation mark is typed like a normal
apostrophe, while the opening quotation mark is typed using the French
\emph{accent grave} on your keyboard (the \emph{accent grave} is the
one going down, as in \emph{frère}).

Note that any punctuation that \emph{semantically} follows quoted
speech goes inside the quotes in American English, but outside in
Britain.  Also, Americans use double quotes first.  Oppose
\begin{quote}
  ``Using `lasers,' we punch a hole in \ldots\ the Ozone Layer,''
  Dr.\ Evil said.
\end{quote}
to
\begin{quote}
  `Using ``lasers'', we punch a hole in \ldots\ the Ozone Layer',
  Dr.\ Evil said.
\end{quote}

\begin{Rule}
  Use hyphens (-), en-dashes (--) and em-dashes (---) correctly.
\end{Rule}

A hyphen is only used in words like `well-known', `$3$-colorable'
etc., or to separate words that continue in the next line (which is
known as hyphenation).  It is entered as a single ASCII hyphen
character (\texttt{-}).

To denote ranges of numbers, chapters, etc., use an en-dash (entered
as two ASCII hyphens \texttt{--}) with no spaces on either side.  For
example, using Equations (1)--(3), we see\ldots

As the equivalent of the German \emph{Gedankenstrich}, use an en-dash
with spaces on both sides -- in the title of Section \ref{sec:list},
it would be wrong to use a hyphen instead of the dash. (Some English
authors use the even longer emdash (---) instead, which is typed as
three subsequent hyphens in \LaTeX. This emdash is used without spaces
around it---like so.)


\section{Spacing}

\begin{Rule}
  \label{rule:no-manual-spacing}
  Do not add spacing manually.
\end{Rule}

You should never use the commands \lstinline-\\- (except within
tabulars and arrays), \lstinline[showspaces=true]-\ - (except to
prevent a sentence-ending space after Dr.\ and such),
\lstinline-\vspace-, \lstinline-\hspace-, etc.  The choices programmed
into \LaTeX{} and this style should cover almost all cases.  Doing it
manually quickly leads to inconsistent spacing, which looks terrible.
Note that this list of commands is by no means conclusive.

\begin{Rule}
  Judiciously insert spacing in maths where it helps.
\end{Rule}

This directly contradicts Rule~\ref{rule:no-manual-spacing}, but in
some cases \TeX{} fails to correctly decide how much spacing is
required.  For example, consider
\begin{displaymath}
  f(a,b) = f(a+b, a-b).
\end{displaymath}
In such cases, inserting a thin math space \lstinline-\,- greatly
increases readability:
\begin{displaymath}
  f(a,b) = f(a+b,\, a-b).
\end{displaymath}

Along similar lines, there are variations of some symbols with
different spacing.  For example, Lagrange's Theorem states that
\(\abs{G}=[G:H]\abs{H}\), but the proof uses a bijection \(f\colon
aH\to bH\).  (Note how the first colon is symmetrically spaced, but
the second is not.)

\begin{Rule}
  Learn when to use \lstinline[showspaces=true]-\ - and
  \lstinline-\@-.
\end{Rule}

Unless you use `french spacing', the space at the end of a sentence is
slightly larger than the normal interword space.

The rule used by \TeX{} is that any space following a period,
exclamation mark or question mark is sentence-ending, except for
periods preceded by an upper-case letter.  Inserting \lstinline-\-
before a space turns it into an interword space, and inserting
\lstinline-\@- before a period makes it sentence-ending.  This means
you should write
\begin{lstlisting}
Prof.\ Dr.\ A. Steger is a member of CADMO\@.
If you want to write a thesis with her, you
should use this template.
\end{lstlisting}
which turns into
\begin{quote}
  Prof.\ Dr.\ A. Steger is a member of CADMO\@.  If you want to write
  a thesis with her, you should use this template.
\end{quote}
The effect becomes more dramatic in lines that are stretched slightly
during justification:
\begin{quote}
  \parbox{\linewidth}{\hbox to \linewidth{%
      Prof.\ Dr.\ A. Steger is a member of CADMO\@.  If you}}
\end{quote}

\begin{Rule}
  Place a non-breaking space (\lstinline-~-) right before references.
\end{Rule}

This is actually a slight simplification of the real rule, which
should invoke common sense.  Place non-breaking spaces where a line
break would look `funny' because it occurs right in the middle of a
construction, especially between a reference type (Chapter) and its
number.


\section{Choice of `fonts'}

Professional typography distinguishes many font attributes, such as
family, size, shape, and weight.  The choice for sectional divisions
and layout elements has been made, but you will still occasionally
want to switch to something else to get the reader's attention.  The
most important rule is very simple.

\begin{Rule}
  When emphasising a short bit of text, use \lstinline-\emph-.
\end{Rule}

In particular, \emph{never} use bold text (\lstinline-\textbf-).
Italics (or Roman type if used within italics) avoids distracting the
eye with the huge blobs of ink in the middle of the text that bold
text so quickly introduces.

Occasionally you will need more notation, for example, a consistent
typeface used to identify algorithms.

\begin{Rule}
  Vary one attribute at a time.
\end{Rule}

For example, for \textsc{WeirdSort} we only changed the shape to small
caps.  Changing two attributes, say, to bold small caps would be
excessive (\LaTeX{} does not even have this particular variation).
The same holds for mathematical notation: the reader can easily
distinguish \(g_n\), \(G(x)\), \(\mathcal{G}\) and \(\mathsf{G}\).

\begin{Rule}
  Never underline or uppercase.
\end{Rule}

No exceptions to this one, unless you are writing your thesis on a
typewriter.  Manually.  Uphill both ways.  In a blizzard.


\section{Displayed equations}

\begin{Rule}
  Insert paragraph breaks \emph{after} displays only where they
  belong.  Never insert paragraph breaks \emph{before} displays.
\end{Rule}

\LaTeX{} translates sequences of more than one linebreak (i.e., what
looks like an empty line in the source code) into a paragraph break in
almost all contexts.  This also happens before and after displays,
where extra spacing is inserted to give a visual indication of the
structure.  Adding a blank line in these places may look nice in the
sources, but compare the resulting display

\begin{displaymath}
  a = b
\end{displaymath}

to the following:
\begin{displaymath}
  a = b
\end{displaymath}
The first display is surrounded by blank lines, but the second is not.
It is bad style to start a paragraph with a display (you should always
tell the reader what the display means first), so the rule follows.

\begin{Rule}
  Never use \lstinline-eqnarray-.
\end{Rule}

It is at the root of most ill-spaced multiline displays.  The
\package{amsmath} package provides better alternatives, such as the
\lstinline-align- family
\begin{align*}
  f(x) &= \sin x, \\
  g(x) &= \cos x,
\end{align*}
and \lstinline-multline- which copes with excessively long equations:
\begin{multline*}
  \def\P{\mathrm P}
  \P\bigl[X_{t_0} \in (z_0, z_0+dz_0],\ldots, X_{t_n}\in(z_n,z_n+dz_n]\bigr]
  \\= \nu(dz_0) K_{t_1}(z_0,dz_1) K_{t_2-t_1}(z_1,dz_2)\cdots
  K_{t_n-t_{n-1}}(z_{n-1},dz_n).
\end{multline*}


\section{Floats}

By default this style provides floating environments for tables and
figures.  The general structure should be as follows:
\begin{lstlisting}
\begin{figure}
  \centering
  % content goes here
  \caption{A short caption}
  \label{some-short-label}
\end{figure}
\end{lstlisting}
Note that the label must follow the caption, otherwise the label will
refer to the surrounding section instead.  Also note that figures
should be captioned at the bottom, and tables at the top.

The whole point of floats is that they, well, \emph{float} to a place
where they fit without interrupting the text body.  This is a frequent
source of confusion and changes; please leave it as is.

\begin{Rule}
  Do not restrict float movement to only `here'
  \textnormal{(\lstinline-h-)}.
\end{Rule}

If you are still tempted, you should avoid the float altogether and
just show the figure or table inline, similar to a displayed equation.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "thesis"
%%% End:

